Reflection from a multi-species material and its transmitted effective wavenumber

We formally deduce closed-form expressions for the transmitted effective wavenumber of a material comprising multiple types of inclusions or particles (multi-species), dispersed in a uniform background medium. The expressions, derived here for the first time, are valid for moderate volume fractions and without restriction on the frequency. We show that the multi-species effective wavenumber is not a straightforward extension of expressions for a single species. Comparisons are drawn with state-of-the-art models in acoustics by presenting numerical results for a concrete and a water-oil emulsion in two dimensions. The limit of when one species is much smaller than the other is also discussed and we determine the background medium felt by the larger species in this limit. Surprisingly, we show that the answer is not the intuitive result predicted by self-consistent multiple scattering theories. The derivation presented here applies to the scalar wave equation with cylindrical or spherical inclusions, with any distribution of sizes, densities, and wave speeds. The reflection coefficient associated with a half-space of multi-species cylindrical inclusions is also formally derived.

==> tex/Intro.tex <==

\section{Summary}
\label{sec:prelude}
Materials comprising mixtures of diverse particles, inclusions, defects or inhomogeneities dispersed inside a background medium arise in a wide range of applications, including
composite materials, emulsions, gases, polymers, foods, and paints. We will refer to these
%
%We are surrounded by fluids, gases and solids, which are essentially a mix of different inclusions. And a highly successful way to measure these materials is to use wave scattering and wave propagation experiments. In practise, the receivers used, in both acoustics and electromagnetism, measure what we call the effective (ensemble average) properties of the medium.
%
\end{fmtext}
\maketitle
%%%%%%%%%%%%%%% End of first page %%%%%%%%%%%%%%%%%%%%%
\noindent
as multi-species materials.
 Of great importance is the ability to characterise these materials and their {\it microstructure}, such as  particle size distribution and volume fractions. One approach to do this is to employ waves, including electromagnetic, acoustic, and elastodynamic waves.
If either the receivers are much larger than the inclusions, or the wavelength is much longer than the inclusions, then the receivers will measure the \textit{ensemble-averaged} properties of the wave~\cite{pinfield_emergence_2013}. This includes the wave speed, attenuation and reflection. Even methods that estimate fluctuations of the wave on smaller scales, such as the averaged intensity, often require the ensemble-averaged wave properties as a first step~\cite{foldy_multiple_1945,tsang_radiative_1987,tsang_dense_2000}. So in order to improve material characterisation, or to design materials with tailored properties, a crucial step is to rigorously calculate the sound speed and attenuation for multi-species materials.


In this paper, we present and formally deduce the effective wavenumber and reflected field of a plane wave scattered by a material comprising different families, or \textit{species}, of particles with distributions of sizes and properties.
The work here differs from the existing literature as our results are not limited to low frequencies and are valid for moderate number density.
% Although we do assume that the matrix and particle material properties are non-dispersive.
This is achieved by extending the methods introduced in~\cite{linton_multiple_2005} for calculating the effective transmission into a half-space of a single species material.

Our approach does not rely on an extinction theorem or the manipulation of divergent integrals or series. The one assumption that is employed is the {\it quasi-crystalline approximation}~\cite{lax_multiple_1951}. For a single species, this approximation is supported by theoretical~\cite{martin_multiple_2008,martin_estimating_2010}, numerical~\cite{chekroun_time-domain_2012}
and experimental~\cite{west_comparison_1994} evidence, however the authors are unaware of any rigorous bounds for the error introduced by this approximation.
\add{We remark that the quasi-crystalline approximation makes no assumption on the material properties, so in principal it is consistent for weak scattering, low or high frequency, or in dense or sparse mixtures. It is also exact when there is only one possible configuration for the particles, for example, when the particle centres lie on the coordinates of a crystal lattice [Lax 1952, where QCA is discussed under (4.3)].}
For simplicity, we also restrict attention to the case of circular cylindrical or spherical particles, although our methods can be extended to the case of general-shaped shaped particles by using Waterman's T-matrix approach \cite{waterman_symmetry_1971,varadan_multiple_1978,mishchenko_t-matrix_1996}, for example.


%\art{ Is it okay that I delete:

%This is done by determining effective parameters and fields that accurately describe and capture the behaviour of ensemble-averaged  fields in the inhomogeneous medium.
%}
% That is, the average sound speed, attenuation, or reflection. This is because the receiver is often much larger than the inclusions and distances between them. Even methods which estimate the fluctuations of the wave on smaller scales, such as the averaged intensity, often require as a first step the effective wave~\cite{foldy_multiple_1945,tsang_radiative_1987,tsang_dense_2000}.


 %for materials with inclusions of different sizes and properties, valid for moderate dense media and without any restriction on the frequency.

In the context of electromagnetic wave scattering, methods for predicting wave propagation and reflection for multi-species material have previously been developed \cite{tsang_radiative_1987,ding_effective_1988,tsang_dense_2000}. These models have been useful for interpreting data from remote sensing, although it appears that such models cannot systematically reproduce experimental results~\cite{tedesco_intercomparison_2006}. In numerous contexts, but particularly in the context of electromagnetics, the standard approach is to employ the Lippman-Schwinger formulation ~\cite{tourin_multiple_2000,sheng_introduction_2006}. However, such a formulation is restrictive as it is not valid for magnetic media in the electromagnetism context or for scatterers with varying density in acoustics, as identified in \cite{martin_acoustic_2003}. Although it is possible to extend the Lippman-Schwinger formulation to account for this effect~\cite{martin_acoustic_2003}, we found it simpler to extend the multiple scattering theory~\cite{fikioris_multiple_1964,foldy_multiple_1945,linton_multiple_2006}.

%\art{ Isn't this exactly what we do? Okay if I remove?

%In particular the approach commonly taken is to first solve the multiple-scattering problem for a single configuration of inclusions and then to ensemble average this solution, following the treatment for the single species case in e.g.\ \cite{fikioris_multiple_1964,foldy_multiple_1945}. However, this approach removes insight on higher-order scattering processes in multi-species media, whereas our approach captures these interactions.
%}

Our approach is also in contrast to coupled-phase theory where the first step is to estimate the ensemble average of the governing equations~\cite{spelt_attenuation_2001}, without explicitly considering multiple-scattering. Although this method can accommodate hydrodynamic interactions and has been extended to polydisperse inclusions (multi-species) it does not completely capture multiple-scattering~\cite{spelt_determination_1999,baudoin_extended_2007}.
%\textbf{\tcr{ART- I have rephrased this para to stress that these methods do not incorporate MST correctly - I assume from your original para that this is true but just check my wording}}.


A suggestion for calculating the multi-species effective wavenumber came from Waterman \& Truell, Equation (3.25a) in the conclusion of \cite{waterman_multiple_1961}. Their suggested formula has been extensively employed in acoustics, see for example \cite{vander_meulen_theoretical_2001,javanaud_experimental_1991,challis_ultrasound_2005}.
 However, their formula is only valid for low frequency and dilute distributions of particles~\cite{linton_multiple_2006}, so it does not properly account for multiple scattering. The approach in  \cite{waterman_multiple_1961} combined with \cite{lloyd_wave_1967} led eventually to the state-of-the-art models for the effective acoustic wavenumber   in colloidal dispersions~\cite{challis_ultrasound_2005}. We numerically compare our results with these authors.


Given an overall particle number density $\nfrac {}$ and background wavenumber  $k$, our main results for a multi-species material comprising \textit{circular cylinders} are the effective transmitted wavenumber:
\begin{equation}
  k_\eff^2 = k^2 - 4 \ii \nfrac {} \ensem{f_\circ}(0) -  4 \ii \nfrac {}^2 \ensem{f_{\circ\circ}}(0)
  + \mathcal O(\nfrac {}^3),
  \label{eqn:wavenumber_results}
\end{equation}
and for an incident wave $u_\inc = \ee^{\ii \alpha x + \ii \beta y}$, with $(\alpha ,\beta) = k(\cos \theta_\inc, \sin \theta_\inc)$, the averaged reflected wave from the inhomogeneous halfspace,
\begin{equation}
 \langle u_\reflect \rangle =  \frac{\nfrac {}}{\alpha^2}\left [
    R_1 + \nfrac {} R_2
  \right]\ee^{-\ii \alpha x + \ii \beta y} + \mathcal O (\nfrac {}^3),
  \label{eqn:reflection_results}
\end{equation}
where
\begin{align}
  & R_1 = \ii \ensem{f_\circ}(\theta_\reflect), \quad \theta_\reflect = \pi - 2 \theta_\inc,
  \label{eqn:R1}
  \\
  & R_2 = \frac{2 \ensem{f_\circ}(0)}{\alpha^2}\left [\frac{\alpha \beta}{k^2}\ensem{f_\circ}'(\theta_\reflect) - \ensem{f_\circ}(\theta_\reflect) \right] + \ii \ensem{f_{\circ\circ}}(\theta_\reflect),
  \label{eqn:R2}
\end{align}
and the functions $\ensem{f_\circ}$ and $\ensem{f_{\circ\circ}}$ are defined in~\eqref{eqns:FarFields} and~\eqref{eqn:MST-pattern}. The formula~\eqref{eqn:reflection_results} is briefly deduced in Section~\ref{eqn:AverageCoefficient}\ref{sec:Reflection},
 and in Figure~\ref{fig:reflect_farfield} we give a pictorial representation, although we stress that the choice $\theta_\reflect = \pi - 2 \theta_\inc$ is not due to a simple geometric argument, but appears from rigorous derivations. From the reflection coefficient~\eqref{eqn:reflection_results} it is possible to choose effective material properties~\cite{caleap_effective_2012}. However, because the reflection coefficient depends on the angle of incidence via $\ensem{f_\circ}(\theta_\reflect)$ and $\ensem{f_{\circ \circ}}(\theta_\reflect)$, it is likely that these effective material properties   change with the angle of incidence.

In the supplementary material we provide a brief self-contained version of these formulas, and the corresponding result for spherical particles, both for a finite number of species. We also provide open source code that implements these formulas, see~\cite{gower_effectivewaves.jl:2017}.
% These results are deduced from the 2D Helmholtz equation~\eqref{eq:governingop}, where for acoustics the pressure $u$ is subject to the boundary conditions~\eqref{eqn:BC}.
For spherical inclusions the effective transmitted acoustic wavenumber becomes,
\begin{align}
   k_\eff^2 = k^2 -\nfrac {} \frac{4 \pi \ii}{k}  \ensem{F_\circ}(0) + \nfrac {}^2 \frac{(4 \pi)^2 }{k^4} \ensem{F_{\circ\circ}}
   + \mathcal O(\nfrac {}^3),
  \label{eqn:SmallNfracSpheres}
\end{align}
where $\ensem{F_\circ}$ and $\ensem{F_{\circ\circ}}$ are functions associated with scattering from the spherical particle and are defined in~\eqref{eqns:SphericalPatterns}. Note that $\ensem{F_{\circ\circ}}$ has no $\theta$ dependency. For a longer discussion of multiple scattering from spheres see \cite{caleap_effective_2012}.

%Expressions for the averaged reflection from a halfspace with multi-species spherical inclusions will follow in another paper; it is beyond the scope of the present study. \tcr{ART - you need more detail here - what sort of details?? At least say that. \textbf{See \cite{caleap_effective_2012} for some details on reflection from spheres.} Agreed}

By developing \textit{multi-species} formulas valid for higher number densities and frequencies, we open up the possibility of characterising and designing a wide  range of advanced materials. The effects of multiple scattering appear only for moderate number density, i.e.\ in the term $\ensem{f_{\circ\circ}}(0)$ in \eqref{eqn:wavenumber_results} and $\ensem{F_{\circ\circ}}$ in \eqref{eqn:SmallNfracSpheres}. One important consequence  of this multiple scattering term  is that a multi-species material can exhibit properties not exhibited by that of the background medium with only one constituent species. We stress that even for just two types of circular cylindrical particles, the effects of multiple scattering are neither intuitive nor easily deduced from the single species case. This becomes apparent in the simple example of a multi-species material where one species is much smaller than the other. In this scenario, we compare our expression for the multi-species effective wavenumber with the state-of-the-art models from acoustics~\cite{challis_ultrasound_2005} and a \textit{self-consistent} type approximation~\cite{sabina_simple_1988,yang_dynamic_2003,kim_generalized_2004}, which can be calculated from the single species formula via an iterative approach: first one \textit{homogenizes} the small particle and background mixture before considering the multiple scattering of the larger particles in the new (homogenized) background medium.
% : first we calculate the effective wavenumber $k_{\eff\cs}$ of a medium with only the smaller specie, then we calculate the effective wavenumber $k_{\eff\cl\cs}$ of a medium with background wavenumber $k_{\eff\cs}$, instead of $k$, and filled with only the larger species.
We show analytically that this naive self-consistent methodology is not even correct in the low-frequency limit. This is then demonstrated numerically for the cases of an emulsion and concrete. \add{Our results are in in-line with \cite{gajdardziska-josifovska_silvermagnesium_1989}, who discuss an effective medium model of a three-phased material in the low-frequency limit.}
% , and also compare the effective wavenumber for a low number fraction multi-species media.

The outline of this paper is as follows. In Section~\ref{sec:Multipole} we describe the exact theory of multiple scattering for $N$ cylinders of any radius, density and sound speed. From there we   calculate the effective (ensemble averaged) equations and apply statistical approximations in Section~\ref{sec:Averaged}.  In Section~\ref{sec:EffectiveWavenumbers} we   deduce the governing system for  the effective wavenumbers at arbitrary total number density and arbitrary frequency, before specialising the result to the case of moderate number fraction and low frequency. In Section~\ref{sec:TwoTypes} we investigate the specific, representative case of  two types of circular cylindrical species   and compare different approximations graphically. To calculate the reflected or transmitted wave we also need the effective amplitude, which we calculate in Section~\ref{eqn:AverageCoefficient} followed by the effective reflected wave. We close in Section~\ref{sec:conclusion}, where we discuss avenues for improvement of the techniques and more general further work.

%we discuss the shortcomings and applications of our multi-species formulas.


==> tex/Percus.tex <==
\section{Pair distribution function}
\label{sec:Percus}
Here we show that for a uniformly distributed particles, the pair distribution function $\chi \to 0$ when the number fraction $\nfrac o \to 0$. In \cite{ding_monte_1992} they discuss how to calculate the pair correlation function $h_{ij}$ defined by
\begin{equation}
h_{ij}(\vec x_i, \vec x_j) =
  \begin{cases}
     -1  \quad &\text{for} \quad R_{ij} < a_{ij}, \\
     \chi(R_{21}| \vec s_1, \vec s_2)  \quad &\text{for} \quad R_{ij} \geq a_{ij}.
  \end{cases}
\en{equation}
using Percus-Yevick approximation, their equations (2-4). In 2D the equations have a similar structure~\cite{adda-bedia_solution_2008}.

In \cite{ding_monte_1992}, $\nfrac \ell$ is the number density of the $\ell-$th type of particle. Assume that $\nfrac \ell = \alpha_\ell \nfrac o$ for some fixed $\alpha_\ell$, implying that $\nfrac \ell \to 0$ as the total number density $\nfrac o \to 0$. That way we write an expansion for small $\nfrac o$
\[
y_{ij}(r) \sim y_{ij}^0(r) + y_{ij}^1(r) \nfrac o.
\]
Substituting the above in \cite{ding_monte_1992} equations (2-3) and then using the result in their equation(2) leads to $y_{ij}^0(r) = 1$, which in turn implies that $\chi^0 = 0$.
% For reference, they use
% \[
% g_{ij}(\vec x_i, \vec x_j) = (1+ \chi(R_{21}| \vec s_1, \vec s_2))H(R_{21} - a_{21}).
% \]


==> tex/ResultsForUniform.tex <==
\subsection{Results for uniformly distributed cylindrical species}
\label{sec:results}
We consider an incident wave $\ee^{\ii \mathbf k \cdot \mathbf x}$ in 2D, with
\begin{gather}
  u_\inc(x,y) = \ee^{\ii \mathbf k \cdot \mathbf x}, \quad \text{with} \quad \mathbf k \cdot \mathbf x = \alpha  x  + \beta y,
\notag \\
  \text{where} \qquad  \alpha = k \cos \theta_\inc, \quad \beta = k \sin \theta_\inc,
  \label{eqns:incident}
\end{gather}
and angle of incidence $\theta_\inc$ from the $x$-axis, exciting a material occupying the halfspace between $0<x$. The halfspace contains $S$ species of cylinders, uniformly distributed each with
\begin{align}
  &\text{number density} \;\; \nfrac j, \quad \text{radius}\;\; a_j,
\notag\\
  &\text{density} \;\; \rho_j, \quad \text{sound speed} \;\; c_j,
\label{properties}
\end{align}
where we use $\nfrac {} = \sum_j \nfrac j$ for the total number density. The background medium has density $\rho$ and sound speed $c$.

For acoustics we solve the 2D scalar wave equation~\eqref{eq:governingop} for the pressure subject to the boundary conditions~\eqref{eqn:BC}. In electromagnetism, we obtain the same system
when the magnetic field is polarised in the direction along the cylinders by replacing $c \mapsto c_0 / n$ and $\rho \mapsto \mu_\mathrm{r}$, where $c_0$ is the speed of light in vacuum, $n$ is the refractive index of the material,  and $\mu_\mathrm{r}$ is the linear magnetic susceptibility. And likewise, when the electric field is polarised along the cylinders, with the replacements $c \mapsto c_0 / n$   and $\rho \mapsto \varepsilon_{r}$, where $\varepsilon_\mathrm{r}$ is the linear electric susceptibility.
% \pagebreak

We can now define the ensemble-average far-field pattern and multiple-scattering pattern,\footnote{Note we introduced the terminology ``multiple-scattering pattern''.}
\begin{align}
  &\ensem{f_\circ}(\theta) = - \sum_{\ell=1}^S  \sum_{n=-\infty}^\infty  \frac{\nfrac \ell}{\nfrac {}} \scatZ_\ell^n \ee^{\ii n \theta},
\\
  &\ensem{f_{\circ\circ}}(\theta) = - \pi  \sum_{\ell,j=1}^S \sum_{m,n=-\infty}^\infty  a_{\ell j}^2 d_{n-m}(k a_{\ell j})  \frac{\nfrac \ell \nfrac j}{\nfrac {}^2}\scatZ_\ell^n \scatZ_j^m \ee^{\ii n \theta},
\end{align}
where $d_m(x) = J_m'(x) H_m'(x) + (1 - (m/x)^2)J_m(x) H_m(x)$, the $J_m$ are Bessel functions, the $H_m$ are Hankel functions of the first kind and $a_{\ell j} > a_\ell + a_j$ is some fixed distance. The  $\scatZ^m_j$ describe the type of scatterer:
\be
\scatZ^m_j = \frac{q_j J_m' (k a_j) J_m ( \gamma k a_j) - J_m (k a_j) J_m' (\gamma k a_j) }{q_j H_m '(k a_j) J_m(\gamma k a_j) - H_m(k a_j) J_m '(\gamma k a_j)} = \scatZ^{-m}_j,
\label{eqn:Zm}
\en

with $q = (\rho_j c_j)/(\rho c)$ and $\gamma = c/c_j$. For instance, taking the limits $q \to 0$ or $q \to \infty$, recovers Dirichlet or Neumann boundary conditions, respectively.

Assuming low number density $\nfrac {}$ (or low volume fraction $\sum_\ell \pi a_\ell^2 \nfrac \ell$), the effective transmitted wavenumber $k_\eff$ becomes
\begin{align}
   k_\eff^2 = k^2 - 4 \ii \nfrac {} \ensem{f_\circ}(0) -  4 \ii \nfrac {}^2 \ensem{f_{\circ\circ}}(0)
   + \mathcal O(\nfrac {}^3),
  \label{eqn:SmallNfracDiscrete}
\end{align}
which is calculated in detail in Section~\ref{sec:EffectiveWavenumbers} for any distribution of species (not just uniform) and we show how to introduce a pair-correlation between the species. The above reduces to \cite{linton_multiple_2005} equation (81) for a single species. This single species formula has been confirmed by several independent methods~\cite{martin_estimating_2010,martin_multiple_2008,chekroun_time-domain_2012,kim_models_2010} in the low frequency limit.

The ensemble-average reflected wave measured at $x <0$ is given by
\begin{equation}
  \ensem{u(x,y)}
   =
  u_\inc(x,y)
  + \frac{\nfrac {}}{\alpha^2}\left [
    R_1 + \nfrac {} R_2
  \right]\ee^{-\ii \alpha x + \ii \beta y} + \mathcal O (\nfrac {}^3),
  \label{eqn:reflection_results}
\end{equation}
where
\begin{align}
  &R_1 = \ii \ensem{f_\circ}(\theta_\reflect), \quad \theta_\reflect = \pi - 2 \theta_\inc,
  \\
  &R_2 = \frac{2 \ensem{f_\circ}(0)}{\alpha^2}\left [\frac{\alpha \beta}{k^2}\ensem{f_\circ}'(\theta_\reflect) - \ensem{f_\circ}(\theta_\reflect) \right] + \ii \ensem{f_{\circ\circ}}(\theta_\reflect),
\end{align}
which is calculated in Section~\ref{sec:Reflection}. The above reduces to \cite{martin_multiple_2011} equations (40-41) for a single species, wherein they show agreement with other known results for a low frequency approximation.

\subsection{Effective wavenumber for multi-species spheres}
\label{sec:Effective3D}

This is the only section where we consider the effective wavenumber in an ensemble of sphere. Meaning that the definitions presented here will not be used anywhere else. The formulas here are deduced by applying the theory we develop in this paper to the results in \cite{linton_multiple_2006}.

\art{Begin deducing formulas.}
Below when I say their equation, I mean an equations in \cite{linton_multiple_2006}. From their equation (4.32), (4.27) and using $b = a_{ij}$ and adding sums over the different species wirghted be their number fraction, we get
\begin{gather*}
k_\eff^2 = k^2 + \nfrac {} \delta_1  + \nfrac {}^2 \delta_2
\\
\delta_2 = \frac{(4 \pi)^4 \ii}{2k^3} \sum_{n=0}^\infty \sum_{p=0}^\infty \sum_q \sum_{i,j=1}^S \frac{\nfrac i \nfrac j}{\nfrac {}^2} \delta_{i,j}^{n,p,q} a_{ij} d_q(k a_{ij}) \scatZ_i^n \scatZ_j^p,
\\
\delta_{i,j}^{n,p,q} =  \sum_{m=-n}^n \sum_{\ell=-p}^p
(-1)^m   Y^m_n(\hat{\vec K})\overline{Y^\ell_p(\hat{\vec K})}
 Y_q^{\ell -m}(\hat{\vec K})\mathcal G(n,m;p,-\ell;q),
\end{gather*}
where $\delta_{i,j}^{n,p,q}$ is similar to their $K_{np}(\vec{\hat K})$, but without the sum in $q$ and without replacing $d_q(x)$ for $in/x$. Then from ther equation (4.34) and below:
\begin{multline*}
\delta_{i,j}^{n,p,q} = \frac{\sqrt{(2n+1)(2p+1)}}{(4 \pi)^{3/2}}  \sqrt{2 q +1} \mathcal G(n,0;p,0;q),
\end{multline*}
which leads to the reduced form
\[
\delta_2 = \frac{(4 \pi)^4 \ii }{2k^3} \sum_{n=0}^\infty \sum_{p=0}^\infty \sum_q \sum_{i,j=1}^S \frac{\nfrac i \nfrac j}{\nfrac {}^2} \frac{\sqrt{(2n+1)(2p+1)}}{(4 \pi)^{3/2}}  \sqrt{2 q +1} \mathcal G(n,0;p,0;q) a_{ij} d_q(k a_{ij}) \scatZ_i^n \scatZ_j^p,
\]
so that $
\delta_2 = \frac{(4 \pi)^2 }{k^4} \ensem{F_{\circ\circ}},
$ with $\ensem{F_{\circ\circ}}$ defined below.
For the formulas below I use $\mathcal G(n,p,q) := \mathcal G(n,0;p,0;q)$.
\art{End deducing formulas.}

For spheres we define the ensemble-average far-field pattern and multiple-scattering pattern,
\begin{align}
  &\ensem{F_\circ}(\theta) = - \sum_{n=0}^\infty  \sum_{i=1}^S (2n+1) \frac{\nfrac i}{\nfrac {}} \scatZs_i^n P_n (\cos \theta ),
\\
  &\ensem{F_{\circ\circ}} = \frac{\ii (4 \pi)^2}{2} \sum_{n=0}^\infty \sum_{p=0}^\infty \sum_q \sum_{i,j=1}^S \frac{\nfrac i \nfrac j}{\nfrac {}^2} \frac{\sqrt{(2n+1)(2p+1)}}{(4 \pi)^{3/2}}  \sqrt{2 q +1} \mathcal G(n,p,q) k a_{ij} d_q(k a_{ij}) \scatZs_i^n \scatZs_j^p,
\notag
\end{align}
where $d_m(x) = x j_m'(x)( x h_m'(x) + h_m(x)) + (x^2 - m(m+1))j_m(x) j_m(x)$, $P_n$ are the Legendre polynomials, $j_m$ are the spherical Bessel functions, $h_m$ are spherical Hankel functions of the first kind  and
\be
\scatZs^m_j = \frac{q_j j_m' (k a_j) j_m ( \gamma k a_j) - j_m (k a_j) j_m' (\gamma k a_j) }{q_j h_m'(k a_j) j_m(\gamma k a_j) - h_m(k a_j) j_m '(\gamma k a_j)} = \scatZs^{-m}_j,
\label{eqn:Zm}
\en
with $q = (\rho_j c_j)/(\rho c)$ and $\gamma = c/c_j$. The $\mathcal G$ is a Gaunt coefficient and is equal to...
% For instance, taking the limits $q \to 0$ or $q \to \infty$, recovers Dirichlet or Neumann boundary conditions, respectively.

Assuming low number density $\nfrac {}$, the effective transmitted wavenumber $k_\eff$ becomes
\begin{align}
   k_\eff^2 = k^2 -\nfrac {} \frac{4 \pi \ii}{k}  \ensem{F_\circ}(0) + \nfrac {}^2 \frac{(4 \pi)^2 }{k^4} \ensem{F_{\circ\circ}}
   + \mathcal O(\nfrac {}^3),
  \label{eqn:SmallNfracDiscreteSpheres}
\end{align}
which is the multi-species finite frequency version of the wavenumber introduced in \cite{lloyd_wave_1967}.


==> tex/table_properties.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l| l|}
  \hline
Background properties: &  wavenumber $k$ \hspace{0.8cm} density $\rho$  \hspace{0.25cm} sound speed $c$
\\ \hline
Specie properties: & number density $\nfrac j$ \hspace{0.1cm} density $\rho_j $
\hspace{0.1cm} sound speed $c_j$  \hspace{0.1cm} radius $a_j$
\\\hline
\multicolumn{2}{|l|}{
  total number density $\nfrac {}$   \hspace{0.2cm}  effective wavenumber $k_\eff$ \hspace{0.2cm} species min. distance $a_{j\ell} > a_j + a_\ell$
}
\\\hline
% 2D Incident wave & $u_\inc(x,y) = \ee^{\ii \mathbf k \cdot \mathbf x} \quad \text{with} \quad \mathbf k \cdot \mathbf x = k x \cos \theta_\inc  + k y \sin \theta_\inc $
\end{tabular}
\label{tab:properties}
\caption{Summary of material properties and notation. The index $j$ refers to properties of the $j$-th species. Note a typical choice for $a_{j\ell}$ is $a_{j\ell} = c (a_j + a_\ell)$, where $c=1.01$.}
\end{table}

